Code Clone Detection based on Event Embedding and Event Dependency

The code clone detection method based on semantic similarity has important value in software engineering tasks (e.g., software evolution, software reuse). Traditional code clone detection technologies pay more attention to the similarity of code at the syntax level, and less attention to the semantic similarity of the code. As a result, candidate codes similar in semantics are ignored. To address this issue, we propose a code clone detection method based on semantic similarity. By treating code as a series of interdependent events that occur continuously, we design a model namely EDAM to encode code semantic information based on event embedding and event dependency. The EDAM model uses the event embedding method to model the execution characteristics of program statements and the data dependence information between all statements. In this way, we can embed the program semantic information into a vector and use the vector to detect codes similar in semantics. Experimental results show that the performance of our EDAM model is superior to state of-the-art open source models for code clone detection.

==> acknowledgement.tex <==
\section{Acknowledgement}\label{section:acknowledgement}
This work was supported in part by the National Key Research and Development Program of China under Grant No. 2018YFB2100805, National Natural Science Foundationof China under the grant No.61962017, 61662019, the Key Research and Development Program of Hainan Province under grant No. ZDYF2020008, Natural Science Foundation of Hainan Province under the grant No. 2019CXTD400, 2019RC088, and grants from State Key Laboratory of Marine Resource Utilization in South China Sea and Key Laboratory of Big Data and Smart Services of Hainan Province.


==> threat.tex <==
\subsection{Threats to Validity}

The initialization of the network parameters and the negative samples selected during the training process will affect the performance of the model. To alleviate the influence of these confounding factors, we will train multiple models and use their average results to evaluate our model.

Uncertain factors in the model training process will also affect the performance of the model. In order to solve this problem and improve the performance of our model, we use a hybrid model to combine the advantages of the two models at the same time and improve the performance of our model.

In experiments, biased dataset may affect the generalization of the results. Therefore, in our experiment, we use the OJClone dataset to train our model. This dataset is an open source dataset containing many OJ questions, and each code fragment in the dataset is submitted by a different person. This means that the diversity of code semantics in the data set is rich, which is an important feature of real-world projects. Therefore, we choose this data set to solve the problem of bias in the data set.

